Subfactors of index less than 5, part 1: the principal graph odometer

In this series of papers we show that there are exactly ten subfactors, other than $A_\infty$ subfactors, of index between 4 and 5. Previously this classification was known up to index $3+\sqrt{3}$. In the first paper we give an analogue of Haagerup's initial classification of subfactors of index less than $3+\sqrt{3}$, showing that any subfactor of index less than 5 must appear in one of a large list of families. These families will be considered separately in the three subsequent papers in this series.

==> documentclasshack.tex <==
%auto-ignore
%%%%%% a hack to make the documentclass name available later %%%
% Thanks to Morten Høgholm. I stole this code from 
% http://groups.google.com/group/comp.text.tex/msg/142306cc7f8acdac
\let\LaTeXdocumentclass\documentclass
\renewcommand*\documentclass[2][]{%
   \newcommand*\ClassName{#2}% for later use
   \LaTeXdocumentclass[#1]{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> pgfsubpic.tex <==
%    pgfsubpic.tex
%    Version 1.1, 25 Dec 2009

%    Copyright 2009 by David Chiang

%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.

%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.

%    You should have received a copy of the GNU General Public License along
%    with this program; if not, write to the Free Software Foundation, Inc.,
%    51 Franklin Street, Fifth Floor, Boston, MA 02110-1301 USA.

% New in version 1.1:
% - the ability to save a subpicture in local variables
% - nodes in subpictures are tracked if the subpicture is placed with arbitrary transforms
% - new \pgffitsubpicture macro to transform a subpicture (preserving aspect) to fit in a desired box

% To do: 
% - speed up interpictureshift hook by promoting subsubpictures

\newdimen\pgf@subpicminx
\newdimen\pgf@subpicminy
\newdimen\pgf@subpicmaxx
\newdimen\pgf@subpicmaxy

% Special virtual node for current subpicture's bounding box
\expandafter\def\csname pgf@sh@ns@current subpicture\endcsname{rectangle}
\expandafter\def\csname pgf@sh@np@current subpicture\endcsname{%
  \def\southwest{\pgfqpoint{\pgf@subpicminx}{\pgf@subpicminy}}%
  \def\northeast{\pgfqpoint{\pgf@subpicmaxx}{\pgf@subpicmaxy}}%
}
\expandafter\def\csname pgf@sh@nt@current subpicture\endcsname{{\pgf@pt@aa}{\pgf@pt@ab}{\pgf@pt@ba}{\pgf@pt@bb}{\the\pgf@pt@x}{\the\pgf@pt@y}} % the transformation at invocation time
\expandafter\def\csname pgf@sh@pi@current subpicture\endcsname{\pgfpictureid}

% Create a pgfpicture inside an hbox for delayed placement
\def\pgfsubpicture{%
\expandafter\global\expandafter\setbox\pgf@hbox=\hbox\bgroup
\pgfinterruptpicture
\pgfpicture
\relax % not sure why. otherwise a curly brace immediately after causes an error
}

\def\endpgfsubpicture{
\global\pgf@subpicminx=\pgf@picminx
\global\pgf@subpicminy=\pgf@picminy
\global\pgf@subpicmaxx=\pgf@picmaxx
\global\pgf@subpicmaxy=\pgf@picmaxy
\global\edef\subpictureid{\pgfpictureid}%
\pgfsetbaseline{\pgf@picminy}%
\endpgfpicture%
\endpgfinterruptpicture%
\egroup
}

% Allocate registers for saving a subpicture. #1 is text, not a control sequence.
\def\pgfnewsubpicture#1{%
\expandafter\newbox\csname pgf@subpic@hbox@#1\endcsname
\expandafter\newdimen\csname pgf@subpic@minx@#1\endcsname
\expandafter\newdimen\csname pgf@subpic@miny@#1\endcsname
\expandafter\newdimen\csname pgf@subpic@maxx@#1\endcsname
\expandafter\newdimen\csname pgf@subpic@maxy@#1\endcsname
}

% saved subpictures are local to the current group
\def\pgfsavesubpicture#1{%
\expandafter\setbox\csname pgf@subpic@hbox@#1\endcsname\copy\pgf@hbox
\csname pgf@subpic@minx@#1\endcsname\pgf@subpicminx
\csname pgf@subpic@miny@#1\endcsname\pgf@subpicminy
\csname pgf@subpic@maxx@#1\endcsname\pgf@subpicmaxx
\csname pgf@subpic@maxy@#1\endcsname\pgf@subpicmaxy
\expandafter\edef\csname pgf@subpic@id@#1\endcsname{\subpictureid}
}

\def\pgfrestoresubpicture#1{%
\edef\act{\global\noexpand\setbox\pgf@hbox\noexpand\copy\csname pgf@subpic@hbox@#1\endcsname}\act
\expandafter\global\expandafter\pgf@subpicminx\csname pgf@subpic@minx@#1\endcsname
\expandafter\global\expandafter\pgf@subpicminy\csname pgf@subpic@miny@#1\endcsname
\expandafter\global\expandafter\pgf@subpicmaxx\csname pgf@subpic@maxx@#1\endcsname
\expandafter\global\expandafter\pgf@subpicmaxy\csname pgf@subpic@maxy@#1\endcsname
\xdef\subpictureid{\csname pgf@subpic@id@#1\endcsname}
}

% Place a previously-created subpicture, lining up its origin with the current origin
\def\pgfplacesubpicture{
\pgfscope
% expand current bounding box to accommodate subpicture
\pgfpathrectanglecorners{\pgfpoint{\the\pgf@subpicminx}{\the\pgf@subpicminy}}{\pgfpoint{\the\pgf@subpicmaxx}{\the\pgf@subpicmaxy}}%
\pgfusepath{use as bounding box}%
%
% make the subpicture a node in the containing picture
\expandafter\gdef\csname pgf@sh@ns@\subpictureid\endcsname{rectangle}
\expandafter\xdef\csname pgf@sh@np@\subpictureid\endcsname{%
  \noexpand\def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@subpicminx}{\the\pgf@subpicminy}}%
  \noexpand\def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@subpicmaxx}{\the\pgf@subpicmaxy}}%
}%
\pgfgettransform\pgf@temp
\expandafter\xdef\csname pgf@sh@nt@\subpictureid\endcsname{\pgf@temp}%
\expandafter\xdef\csname pgf@sh@pi@\subpictureid\endcsname{\pgfpictureid}%
%
% align origin of subpicture with origin
\pgftransformshift{\pgfpoint{\the\pgf@subpicminx}{\the\pgf@subpicminy}}%
\pgfqboxsynced{\pgf@hbox}%
\endpgfscope
}

% Hook onto existing macro \pgf@shape@interpictureshift.
% This is called whenever we look up an anchor of a node.
% This hook recursively checks to see if the node's picture
% is a subpicture of another, and if so, adjusts its position accordingly.

% This is slow. It makes drawing trees O(n^2) in the depth of the tree.
% The alternative is to store, for each picture, a list of the nodes
% inside it. But this way doesn't require us to hijack \pgfnode, and
% is robust to re-placement of a subpicture. A compromise would be
% to store, for each picture, a list of the *subpictures* inside it.

\let\orig@pgf@shape@interpictureshift\pgf@shape@interpictureshift
\def\unwind@subpic#1{%
% is #1 the current picture?
\edef\subpicid{#1}%
\ifx\subpicid\pgfpictureid
% yes, we're done
\else
% does #1 have a parent picture?
\expandafter\ifx\csname pgf@sh@pi@#1\endcsname\relax
% no, the original node was not inside the current picture
\fallback
\else
% yes, apply transform and move up to parent picture
{%
  \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
  \pgf@pos@transform{\pgf@x}{\pgf@y}%
  \global\pgf@x=\pgf@x
  \global\pgf@y=\pgf@y
}%
\unwind@subpic{\csname pgf@sh@pi@#1\endcsname}%
\fi
\fi
}
\def\pgf@shape@interpictureshift#1{%
\edef\fallback{\pgf@x=\the\pgf@x\pgf@y=\the\pgf@y\noexpand\orig@pgf@shape@interpictureshift{#1}}%
\unwind@subpic{\csname pgf@sh@pi@#1\endcsname}%
}

% \pgffitsubpicture{sw}{ne}
% Make the subpicture fit in the rectangle from sw to ne, preserving its aspect ratio.
\def\pgffitsubpicture#1#2{%
% current size
\pgfpointdiff{\pgfpointanchor{current subpicture}{south west}}{\pgfpointanchor{current subpicture}{north east}}%
\pgf@xa=\pgf@x \pgf@ya=\pgf@y
% desired size
\pgf@process{\pgfpointdiff{#1}{#2}}%
\pgf@xb=\pgf@x \pgf@yb=\pgf@y
\pgfmathparse{min(\pgf@xb/\pgf@xa,\pgf@yb/\pgf@ya)}%
\pgfmathparse{min(1,\pgfmathresult)}%
\pgftransformscale{\pgfmathresult}%
%
% current position
\pgfpointanchor{current subpicture}{center}%
\pgf@xa=\pgf@x \pgf@ya=\pgf@y
% desired position
% we scaled transform, so apply reverse scaling to argument
\pgfmathparse{1/\pgfmathresult}%
\pgf@process{\pgfpointscale{\pgfmathresult}{\pgfpointlineattime{0.5}{#1}{#2}}}%
\pgf@xb=\pgf@x \pgf@yb=\pgf@y
\pgfpointdiff{\pgfpoint{\pgf@xa}{\pgf@ya}}{\pgfpoint{\pgf@xb}{\pgf@yb}}%
\pgftransformshift{\pgfpoint{\pgf@x}{\pgf@y}}%
}

% utility functions -- not currently used

\def\pgfnodedelete#1{%
\expandafter\global\expandafter\let\csname pgf@sh@ns@#1\endcsname\relax
\expandafter\global\expandafter\let\csname pgf@sh@np@#1\endcsname\relax
\expandafter\global\expandafter\let\csname pgf@sh@nt@#1\endcsname\relax
\expandafter\global\expandafter\let\csname pgf@sh@pi@#1\endcsname\relax
\expandafter\global\expandafter\let\csname pgf@sh@ma@#1\endcsname\relax
}

\def\pgfnodeifexists#1#2#3{%
\expandafter\ifx\csname pgf@sh@ns@#1\endcsname\relax#3\else#2\fi
}



==> pgftree.tex <==
%    pgftree.tex
%    Version 1.1, 25 Dec 2009

%    Copyright 2009 by David Chiang

%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.

%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.

%    You should have received a copy of the GNU General Public License along
%    with this program; if not, write to the Free Software Foundation, Inc.,
%    51 Franklin Street, Fifth Floor, Boston, MA 02110-1301 USA.

% New in version 1.1:
% - major restructuring to not do arbitrary nesting of subpicture environments
% - sideways trees

% To do:
% - trees with all leaves at same level
% - if \nodename does not exist as desired, wrap inside a rectangle node
% - don't use pgfsubpic internals

\newdimen\levelsep \levelsep=30pt
\newdimen\subtreesep \subtreesep=2pt

\def\leveldirection{down}
\def\siblingdirection{right}

% definitions of growing directions
\def\pgftree@levelshift{\csname pgftree@levelshift@\leveldirection\endcsname}
\def\pgftree@parentanchor{\csname pgftree@parentanchor@\leveldirection\endcsname}
\def\pgftree@childanchor{\csname pgftree@childanchor@\leveldirection\endcsname}
% these assume that the current subpicture is the child
\def\pgftree@presiblingshift{\csname pgftree@presiblingshift@\siblingdirection\endcsname}
\def\pgftree@postsiblingshift{\csname pgftree@postsiblingshift@\siblingdirection\endcsname}

\def\pgftree@levelshift@down{\pgfpoint{0}{-\levelsep}}
\def\pgftree@parentanchor@down{south}
\def\pgftree@childanchor@down{north}

\def\pgftree@levelshift@up{\pgfpoint{0}{\levelsep}}
\def\pgftree@parentanchor@up{north}
\def\pgftree@childanchor@up{south}

\def\pgftree@levelshift@right{\pgfpoint{\levelsep}{0}}
\def\pgftree@parentanchor@right{east}
\def\pgftree@childanchor@right{west}

\def\pgftree@levelshift@left{\pgfpoint{-\levelsep}{0}}
\def\pgftree@parentanchor@left{west}
\def\pgftree@childanchor@left{east}

\def\pgftree@presiblingshift@right{\pgf@process{\pgf@x-\pgf@subpicminx \advance\pgf@x\subtreesep \pgf@y 0pt}}
\def\pgftree@postsiblingshift@right{\pgf@process{\pgf@x\pgf@subpicmaxx \pgf@y 0pt}}

\def\pgftree@presiblingshift@left{\pgf@process{\pgf@x-\pgf@subpicmaxx \advance\pgf@x-\subtreesep \pgf@y 0pt}}
\def\pgftree@postsiblingshift@left{\pgf@process{\pgf@x\pgf@subpicminx \pgf@y 0pt}}

\def\pgftree@presiblingshift@up{\pgf@process{\pgf@x 0pt \pgf@y-\pgf@subpicminy \advance\pgf@y\subtreesep}}
\def\pgftree@postsiblingshift@up{\pgf@process{\pgf@x 0pt \pgf@y\pgf@subpicmaxy}}

\def\pgftree@presiblingshift@down{\pgf@process{\pgf@x 0pt \pgf@y-\pgf@subpicmaxy \advance\pgf@y-\subtreesep}}
\def\pgftree@postsiblingshift@down{\pgf@process{\pgf@x 0pt \pgf@y\pgf@subpicminy}}

% for convenience if you are using \pgftree directly
\def\drawnode#1{\pgfnode{rectangle}{base}{#1}{\nodename}{\pgfusepath{discard}}}
\def\drawedge{%
\pgfpathmoveto{\pgfpointanchor{\parentnodename}{\pgftree@parentanchor}}%
\pgfpathlineto{\pgfpointanchor{\nodename}{\pgftree@childanchor}}%
\pgfusepath{stroke}}

% local variables that we need to assign to inside a \pgfforeach
\newdimen\pgftree@childx
\newdimen\pgftree@savechildx
\newdimen\pgftree@childy
\newdimen\pgftree@savechildy
\newcount\pgftree@childi
\newcount\pgftree@savechildi

%%% \pgftree{subtree}

\def\pgftree#1{%
\def\nodename{r}%
#1
\pgfplacesubpicture
}

%%% \pgfsubtree{root}{subtrees}
% The first argument draws the root node using PGF/TikZ commands.
% The node must be named \nodename.

% The second argument is an even-length sequence of tokens.
% Token 2n-1 in the sequence draws the nth edge. It should draw an edge from \parentnodename to \nodename.
% Token 2n in the sequence draws the nth subtree. Its root must be named \nodename.

\pgfnewsubpicture{children}
\pgfnewsubpicture{child}
\newdimen\pgftree@lastchildx
\newdimen\pgftree@lastchildy

\def\pgfsubtree#1#2{%
\let\parentnodename\nodename
\pgftree@savechildx=\pgftree@childx
\pgftree@savechildy=\pgftree@childy
\pgftree@savechildi=\pgftree@childi
% Build subpicture with all the children and their subtrees. Save it in "children"
{\pgftree@childx=0pt%
\pgftree@childy=0pt%
\pgftree@childi=0%
\process@children #2}%
\ifnum\pgftree@childi>0%
\begin{pgfsubpicture}%
% Create root node
#1
% Place children
% move down \levelsep
{\pgftransformshift{\pgftree@levelshift}%
% center so that parent is midway between origins of first and last children
\pgftransformshift{\pgfpointscale{-0.5}{\pgfpoint{\the\pgftree@childx}{\the\pgftree@childy}}}%
\pgfplacesubpicture}
% Draw the edges
{\pgftree@childi=0%
\process@edges #2}%
\end{pgfsubpicture}%
\else % leaf node
\begin{pgfsubpicture}%
#1
\end{pgfsubpicture}%
\fi
\global\pgftree@childi=\pgftree@savechildi
\global\pgftree@childx=\pgftree@savechildx
\global\pgftree@childy=\pgftree@savechildy
}

\def\process@children{%
\pgfutil@ifnextchar\egroup
{% No more children, step back to origin of last child
\global\pgftree@childx\pgftree@lastchildx
\global\pgftree@childy\pgftree@lastchildy
\global\pgftree@childi\pgftree@childi
\pgfrestoresubpicture{children}% pass children back to caller
}%
{\@process@children}%
}
\def\@process@children#1#2{% #1 is the edge, #2 is the child
% Build the current child and save it as "child"
{\edef\nodename{\parentnodename-\the\pgftree@childi}%
#2}%
\pgfsavesubpicture{child}%
\begin{pgfsubpicture}
% Place previous children (if any)
\ifnum\pgftree@childi>0%
\pgfrestoresubpicture{children}%
\pgfplacesubpicture
\fi
% Place current child
\pgfrestoresubpicture{child}%
\ifnum\pgftree@childi>0% the first child is always at 0
\pgftree@presiblingshift \global\advance\pgftree@childx\pgf@x \global\advance\pgftree@childy\pgf@y
\fi
\global\pgftree@lastchildx\pgftree@childx
\global\pgftree@lastchildy\pgftree@childy
{\pgftransformshift{\pgfpoint{\the\pgftree@childx}{\the\pgftree@childy}}%
\pgfplacesubpicture}%
\pgftree@postsiblingshift \global\advance\pgftree@childx\pgf@x \global\advance\pgftree@childy\pgf@y
\end{pgfsubpicture}%
% Save the augmented row of children back into "children"
\pgfsavesubpicture{children}%
\advance\pgftree@childi by 1%
\process@children
}

\def\process@edges{%
\pgfutil@ifnextchar\egroup
{}%
{\@process@edges}%
}
\def\@process@edges#1#2{%
\edef\nodename{\parentnodename-\the\pgftree@childi}%
#1%
\advance\pgftree@childi by 1%
\process@edges
}

\def\subtreeof#1{%
% the subpicture which contains a node also contains exactly its subtree
\csname pgf@sh@pi@#1\endcsname
}


==> text/tree10.tex <==
%!TEX root = ../index5-1.tex
\hspace{-2cm}
\scalebox{0.72}{
\begin{tikzpicture}
[
level 1/.style={level distance=46mm, sibling distance=40mm,nodes={draw, fill=white, rectangle, rounded corners}},
level 2/.style={level distance=52mm, sibling distance=20mm},
level 3/.style={level distance=58mm, sibling distance=25mm},
level 4/.style={level distance=64mm},
grow=right]\node[draw, fill=white, rectangle, rounded corners] {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1duals1v1v1x2}\\\bigraph{bwd1v1v1v1p1v1x0p1x0duals1v1v1x2}\end{array}$\ref{bwd1v1v1v1p1v1x0p0x1v1x0p0x1duals1v1v1x2v2x1}}
child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x1duals1v1v1x2v1}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1duals1v1v1x2v1x2}\end{array}$\ref{bwd1v1v1v1p1v1x0p0x1v1x1duals1v1v1x2v1}}
child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x1v1duals1v1v1x2v1}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1v1x1duals1v1v1x2v1x2}\end{array}$\ref{bwd1v1v1v1p1v1x0p0x1v1x1v1v1duals1v1v1x2v1v1}}
}}child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p1x0p0x1p0x1duals1v1v1x2v1x3x2x4}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1duals1v1v1x2v1x2}\end{array}$}
child {node [fill=red!30]{$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p1x0p0x1p0x1v0x1x0x0p0x0x1x0duals1v1v1x2v1x3x2x4}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1v0x1p1x0duals1v1v1x2v1x2}\end{array}$}
}child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p1x0p0x1p0x1v1x0x0x0p0x1x0x0p0x0x1x0p0x0x0x1duals1v1v1x2v1x3x2x4}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1v1x0p0x1p1x0p0x1duals1v1v1x2v1x2}\end{array}$}
}child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p1x0p0x1p0x1v0x1x0x0p0x0x1x0p0x0x0x1duals1v1v1x2v1x3x2x4}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1v0x1p1x0p0x1duals1v1v1x2v1x2}\end{array}$}
child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p1x0p0x1p0x1v0x1x0x0p0x0x1x0p0x0x0x1v1x0x0p1x0x0p0x1x0p0x0x1duals1v1v1x2v1x3x2x4v1x4x3x2}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1v0x1p1x0p0x1v1x0x0p0x1x0duals1v1v1x2v1x2v2x1}\end{array}$}
child {node [fill=red!30]{$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p1x0p0x1p0x1v0x1x0x0p0x0x1x0p0x0x0x1v1x0x0p1x0x0p0x1x0p0x0x1v1x0x0x0p0x0x1x0p0x0x0x1duals1v1v1x2v1x3x2x4v1x4x3x2}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1v0x1p1x0p0x1v1x0x0p0x1x0v0x1p1x0p0x1duals1v1v1x2v1x2v2x1}\end{array}$}
}}child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p1x0p0x1p0x1v0x1x0x0p0x0x1x0p0x0x0x1v1x0x0p1x0x0p0x1x0p0x0x1p0x0x1duals1v1v1x2v1x3x2x4v1x4x3x2x5}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1v0x1p1x0p0x1v1x0x0p0x1x0p0x0x1duals1v1v1x2v1x2v2x1x3}\end{array}$}
}child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p1x0p0x1p0x1v0x1x0x0p0x0x1x0p0x0x0x1v1x0x1p0x1x0duals1v1v1x2v1x3x2x4v1x2}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1v0x1p1x0p0x1v1x0x0p0x1x0p0x0x1duals1v1v1x2v1x2v2x1x3}\end{array}$}
}}}child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p0x1p0x1p0x1duals1v1v1x2v2x1x3x4}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v0x1p0x1duals1v1v1x2v1x2}\end{array}$}
child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p0x1p0x1p0x1v1x0x0x0p1x0x0x0duals1v1v1x2v2x1x3x4}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v0x1p0x1v0x1p1x0duals1v1v1x2v1x2}\end{array}$\ref{bwd1v1v1v1p1v1x0p0x1v1x0p0x1p0x1p0x1v1x0x0x0p1x0x0x0v1x0p0x1duals1v1v1x2v2x1x3x4v1x2}}
}}child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x1p0x1duals1v1v1x2v1x2}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1p0x1duals1v1v1x2v1x2x3}\end{array}$\ref{bwd1v1v1v1p1v1x0p0x1v1x1p0x1duals1v1v1x2v1x2}}
child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x1p0x1v0x1duals1v1v1x2v1x2}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1p0x1v0x0x1duals1v1v1x2v1x2x3}\end{array}$\ref{bwd1v1v1v1p1v1x0p0x1v1x1p0x1v0x1duals1v1v1x2v1x2}}
child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x1p0x1v0x1v1duals1v1v1x2v1x2v1}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1p0x1v0x0x1v1duals1v1v1x2v1x2x3v1}\end{array}$\ref{bwd1v1v1v1p1v1x0p0x1v1x1p0x1v0x1v1duals1v1v1x2v1x2v1}}
}}}child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p0x1p0x1duals1v1v1x2v2x1x3}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v0x1duals1v1v1x2v1}\end{array}$}
child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p0x1p0x1v1x0x0duals1v1v1x2v2x1x3}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v0x1v1duals1v1v1x2v1}\end{array}$\ref{bwd1v1v1v1p1v1x0p0x1v1x0p0x1p0x1v1x0x0v1duals1v1v1x2v2x1x3v1}}
}child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p0x1p0x1v1x0x0p0x0x1p0x0x1duals1v1v1x2v2x1x3}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v0x1v1p1p1duals1v1v1x2v1}\end{array}$\ref{bwd1v1v1v1p1v1x0p0x1v1x0p0x1p0x1v1x0x0p0x0x1p0x0x1v1x0x0p1x0x0p1x0x0p0x1x0p0x0x1duals1v1v1x2v2x1x3v1x4x5x2x3}}
}child {node [fill=red!30]{$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p0x1p0x1v1x0x0p0x0x1duals1v1v1x2v2x1x3}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v0x1v1p1duals1v1v1x2v1}\end{array}$}
}}child {node {$\begin{array}{c}\bigraph{bwd1v1v1v1p1v1x0p0x1v1x0p1x0p0x1p0x1p0x1duals1v1v1x2v1x3x2x4x5}\\\bigraph{bwd1v1v1v1p1v1x0p1x0v1x0p0x1p0x1duals1v1v1x2v1x2x3}\end{array}$}
};
\end{tikzpicture}
}


==> tikz-qtree.tex <==
%    tikz-qtree.tex
%    Version 1.1, 25 Dec 2009

%    Copyright (C) 2002, 2009 by David Chiang

%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.

%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.

%    You should have received a copy of the GNU General Public License along
%    with this program; if not, write to the Free Software Foundation, Inc.,
%    51 Franklin Street, Fifth Floor, Boston, MA 02110-1301 USA.

% New in version 1.1:

% - sideways trees

%% These macros facilitate building up an object recursively before
%% putting it into the input stream.

\newtoks\@result
\def\@call#1#2{\let\@cont=#2\bgroup\@result={}#1}
\def\@return{\global\@result=\@result\egroup\@cont}

\def\@ifequal#1#2{\edef\testa{#1}\edef\testb{#2}\ifx\testa\testb}

%% scan a tree: this just scans a subtree and then puts it onto the
%% input stream

\def\Tree{\@call\@subtree\@Tree}
\def\@Tree{%
%\showthe\@result %debug
\ifpgfpicture % is there a test for tikzpicture?
\pgftree{\the\@result}%
\else
\tikzpicture[baseline]\pgftree{\the\@result}\endtikzpicture
\fi
}

%% scan a subtree
\newtoks\child@list
\newtoks\root@node

\def\@subtree[{%
\root@node={}%
\pgfutil@ifnextchar.{\@call\@interior\@@subtree}{\@@@subtree}}
\def\@@subtree{%
\root@node=\@result
\@@@subtree
}
\def\@@@subtree{%
\@call\@children\@@@@subtree
}
\def\@@@@subtree]{%
\child@list=\@result
\pgfutil@ifnextchar.{\@call\@interior\@@@@@subtree}{\@@@@@@subtree}}
\def\@@@@@subtree{%
%%% Check for mismatch.
\@ifequal{\the\root@node}{\pgfutil@empty}%
  \root@node=\@result
\fi
\@ifequal{\the\root@node}{\the\@result}\else
  \message{Warning: mismatched labels, \the\root@node{} and \the\@result.}%
\fi
\@@@@@@subtree
}
\def\@@@@@@subtree{%
\@ifequal{\the\root@node}{\pgfutil@empty}
\edef\act{\noexpand\@result={\noexpand\pgfsubtree{\noexpand\path coordinate (\noexpand\nodename);}{\the\child@list}}}%
\else
\edef\act{\noexpand\@result={\noexpand\pgfsubtree{\the\root@node}{\the\child@list}}}%
\fi
\act
\@return}

%% scan a sequence of subtrees or leaves

\newif\ifscanned@edge

\def\@children{%
\scanned@edgefalse
\child@list{}%
\@@children}
\def\@@children{%
\pgfutil@ifnextchar]{\@result\child@list\@return}{% end of children
\pgfutil@ifnextchar\edge{% explicit edge
\ifscanned@edge
\message{Warning: more than one edge given for a single child}\let\next\@@children % ignore
\else
\scanned@edgetrue\let\next\@@@children
\fi
\@call\@edge\next}{%
% else, a real node is next
\ifscanned@edge\else % no explicit edge, supply default
\expandafter\child@list\expandafter{\the\child@list{\edge@adapter{}}}%
\fi
\scanned@edgefalse
\pgfutil@ifnextchar[{\@call\@subtree\@@@children}% subtree
{\@call\@leaf\@@@children} % leaf
}}}
\def\@@@children{%
% wrap child inside curly braces
\expandafter\@result\expandafter{\expandafter{\the\@result}}
\edef\act{\noexpand\child@list{\the\child@list \the\@result}}\act
\@@children
}

\def\@interior.{\@result{\node[alias=\nodename][every tree node,every internal node]}\@label}

\def\@leaf{\@call\@label\@@leaf}
\def\@@leaf{\edef\act{\noexpand\@result{\noexpand\pgfsubtree{\noexpand\node[alias=\noexpand\nodename][every tree node,every leaf node]\the\@result}{}}}\act\@return}

\def\@edge\edge #1;{%
\@result{\edge@adapter{#1}}%
\@return}
\def\edge@adapter#1{%
\let\tikzparentnode\parentnodename
\let\tikzchildnode\nodename
\path edge from parent #1;%
}

% a label is either text or PGF/TikZ code starting with \node
\def\@label{\pgfutil@ifnextchar\node{\@litlabel}{\@@label}}
\def\@@label#1 {%
\expandafter\@result\expandafter{\the\@result{#1};}%
\@return}

% try to copy \node command into \@result without stripping braces
\def\@litlabel\node{\@@litlabel}
\def\@@litlabel{\pgfutil@ifnextchar\bgroup{\@@@litlabel}{\@@@@litlabel}}
\def\@@@litlabel#1{\expandafter\@result\expandafter{\the\@result {#1}}\@@litlabel}
\def\@@@@litlabel#1;{\expandafter\@result\expandafter{\the\@result #1;}\@return}

% predefined edges

\def\tree@edge#1#2{(#1.\pgftree@parentanchor) -- (#2.\pgftree@childanchor)}

\def\roof@edge#1#2{\csname roof@edge@\leveldirection\endcsname{#1}{#2}}
\def\roof@edge@down#1#2{(#1.south) -- (#2.north west) -- (#2.north east) -- cycle}
\def\roof@edge@up#1#2{(#1.north) -- (#2.south west) -- (#2.south east) -- cycle}
\def\roof@edge@left#1#2{(#1.west) -- (#2.north east) -- (#2.south east) -- cycle}
\def\roof@edge@right#1#2{(#1.east) -- (#2.north west) -- (#2.south west) -- cycle}

%%% Options

\tikzoption{level distance}{\pgfmathsetlength\levelsep{#1}}
\tikzoption{sibling distance}{\pgfmathsetlength\subtreesep{#1}} % different semantics

% I don't really like this scheme
\tikzoption{grow}{\csname grow@#1\endcsname}
\tikzoption{grow'}{\csname growprime@#1\endcsname}
\def\grow@up{\def\leveldirection{up}\def\siblingdirection{left}}
\def\grow@down{\def\leveldirection{down}\def\siblingdirection{right}}
\def\growprime@up{\def\leveldirection{up}\def\siblingdirection{right}}
\def\growprime@down{\def\leveldirection{down}\def\siblingdirection{left}}
\def\grow@left{\def\leveldirection{left}\def\siblingdirection{down}}
\def\grow@right{\def\leveldirection{right}\def\siblingdirection{up}}
\def\growprime@left{\def\leveldirection{left}\def\siblingdirection{up}}
\def\growprime@right{\def\leveldirection{right}\def\siblingdirection{down}}

% defaults appropriate for linguistic trees
\tikzset{every tree node/.style={anchor=base}}
\tikzset{every leaf node/.style={}}
\tikzset{every internal node/.style={}}
\def\tikz@edge@to@parent@path{\tree@edge{\tikzparentnode}{\tikzchildnode}}

% predefined roof style
\tikzset{roof/.style={edge from parent path=\roof@edge{\tikzparentnode}{\tikzchildnode}}}


